ViTO: Vision Transformer-Operator

We combine vision transformers with operator learning to solve diverse inverse problems described by partial differential equations (PDEs). Our approach, named ViTO, combines a U-Net based architecture with a vision transformer. We apply ViTO to solve inverse PDE problems of increasing complexity, namely for the wave equation, the Navier-Stokes equations and the Darcy equation. We focus on the more challenging case of super-resolution, where the input dataset for the inverse problem is at a significantly coarser resolution than the output. The results we obtain are comparable or exceed the leading operator network benchmarks in terms of accuracy. Furthermore, ViTO`s architecture has a small number of trainable parameters (less than 10% of the leading competitor), resulting in a performance speed-up of over 5x when averaged over the various test cases.

==> background.tex <==
\section{Related work}

Several studies have been conducted by the SciML community for both forward and inverse problems. A notable advancement are the Physics-Informed Neural Networks (PINNs), invented by Raissi \textit{et al.} \cite{}. In PINNs, one designs two loss terms that are used simultaneously as the unified target function of the network. The first is the data loss, which operates on the known data, often called the ground truth. For the forward problems this data is usually gathered from the initial and boundary conditions, while for the inverse problem it is gathered from either the sensor measurement, the final state, the medium properties, a combination of the aforementioned, etc. The second loss term enforces the known physics about the problem. One can compute the gradients of the network, hence the derivatives in the different dimensions, and create a loss term by implicitly summing the partial derivatives that compose the equation for the physical model. By using the combination of the two loss terms, PINNs are able to correctly infer the solution of a certain PDE with high accuracy. In addition, they receive a point in time and space and produce the solution at that point, so they are not bound to a mesh. The drawbacks of PINNs are that they are problem specific, meaning that any change of the problem conditions requires training a new PINN which is a costly procedure.

The literature is offers many implementations of PINNs in different forward scenarios, such as mechanics \cite{}, acoustics \cite{}, tomography \cite{}, etc. However, not many PINN papers exist for inverse problems. In \cite{} the authors show how a PINN can be used to recover the wave propagation speed (medium property) using a few measurement of the acoustic scattered wave. In \cite{}, a method that combines Time Reversal \cite{} with a PINN is proposed for finding the source that started the emission of acoustic waves, and similar concepts have been used for identifying and locating a scatterer \cite{}.

Another important factor when dealing with SciML computations in general ,and specifically with inverse problems, is that we often approximate a solution to a problem on a discrete grid. That leads to issues such as the \textit{inverse crime} \cite{}, where one uses the same setup (usually a mesh) for both the forward and the inverse problems solvers. In addition, when dealing with an inverse problem, one does not have data recorded in every point of the domain (especially since the real-world scenario is assumed continuous). Therefore, one tries to reconstruct the solution of the inverse problem using a much more coarse discretization than the theoretical one, a situation which is often referred to as \textit{super resolution} (SR). Methods for SR \cite{} have been investigated throughout the years \cite{}, including ML based methods \cite{}. To emphasize the challenge of SR, an example could be finding an underground movement  e.g. of tectonic plates (geophysics) using recordings from few seismic sensors spread at multiple cities in the country. If one is interested in a solution that is accurate up to, say a few meters, a solution may not be possible.

Vision transformers with examples from classical use cases like CIFAR and medical imaging.

Following the revolution in NLP after the invention of transformers, the ViT, invented by Dosovitskiy \textit{et al.} \cite{}, is the latest advancement for imaging tasks. The proposed ViT architecture splits the image into small patches and translates each patch into a token using linear projections. The tokens that represent the image are then pushed into a transformer. In their paper, the authors demonstrate how the ViT outperforms the SOTA methods for image classifications, including ImageNet \cite{}, CIFAR \cite{}, Oxford pets and flowers \cite{}, and VTAB \cite{}. In addition, the benchmark ViT model is up to four times more efficient than the SOTA methods used as reference. The ViT can also be used in many different fields. In \cite{} the authors used a ViT for X-ray image classification, while in \cite{} it was used for unsupervised volumetric medical image registration. The capabilities of the ViT are vast and it is being currently adopted in various areas of research.

Operator learning has been a accelerating in recent years. The first operator learning method was invented by Lu \textit{et al.}, named the Deep Operator Network (DeepONet) \cite{}. The DeepONet is composed from a branch and a trunk. The branch learns the input function space of the operator, while the trunk learns the space of functions onto which the output is projected. By multiplying the branch with the trunk, the projection provides a representation of the output function space. Another popular invention is the Fourier Neural Operator \cite{}, which is based on a Fourier space kernel. The operator networks do not need to know the physics (unlike their PINN counterparts), and when changing the problem conditions no further training is needed. Using operator networks for inverse problems is natural, since one can train an operator network for many different problems and conditions and exploit the generalization capabilities for finding the solution for a new case. In \cite{}, the authors  demonstrate how to use downstream measurements and DeepONet for the inverse problem of determining the original perturbation of instability waves in high-speed boundary layers. The main drawback of operator networks is that they require a large amount of data for training, which may not be available especially when dealing with inverse problems.


There have been attempts to use transformers for operator learning. In \cite{} the authors use transformers to approximate \emph{forward} solutions of PDEs with operator learning. They propose an innovative way for choosing the collocation points and iterate through time to find the solution at those points. The attention mechanism is split in such a way that the query, key and value are split into different parts of the forward pass and is implemented as a multi-layer perceptron (MLP). \panos{I'm not sure about the previous sentence, something is missing} The latent encoding, which is the outcome of the combination of the three components is the embedding of the coordinates used for the spatio-temporal input of the PDE. In \cite{} the author presents a method to combine FNO with attention to improve the performance for PDE solutions, ny replacing the softmax (often used in transformers especially in classification) with a linear variant of it that does not involve normalization.

==> introduction_old.tex <==
\section{Introduction}

GK: THE INTRODUCTION IS OFF THE MARK. THE FRST PART IS NOT NEEDED.
TALK ABOUT THE HISTORY OF NEURAL OPERATORS and GIVE REFERENCES. THEN WHY NEURAL OPERATORS AND WHAT IS MISSING OR CAN BE IMPROVED. THEN, WHAT IS THE PURPOSE OF THIS PAPER. Geneal blah blas are useless, go directly to the point!
MERGE SECTIONS 1 and 2.
\panos{I'll work on merging 1 and 2 and condensing}

The field of scientific machine learnig (SciML) has been growing rapidly in recent years. Many problems in physics \cite{}, biology \cite{}, chemistry \cite{}, geophysics \cite{}, etc., can be formulated as data driven problems. The accelerated research of artificial intelligence has produced many new techniques for achieving highly accurate classification and regression models. Many of these state-of-the-art (SOTA) methods can be applied for scientific computations. Authors study innovative ways to incorporate the scientific knowledge of the process (mathematical formulation of physics processes, models of biological components, chemical reaction, etc.), into a machine learning algorithm that trains on observations (input and output data samples). By combining the two methodologies, more accurate results are achieved. Another methodology is to completely replace the scientific models with learning machines, that can operate solely on data and approximate the solution of the scientific problem. In this paper we propose such a method. \panos{This sounds a bit contradicting with the previous statement that people are trying to combine scientific models with data. It's as if we are throwing away scientific models when we have said that they are a good thing. I think we should rephrase.}

When modeling a physical experiment we usually find one of two scenarios interesting. The first scenario is the \textit{forward problem}, when given a set of conditions, one attempts to simulate the physical process. For example, given an initial source, find the acoustic wave amplitude in the ocean after some time. The second scenario is the opposite one, called the \textit{inverse problem}. Given the state of the physical experiment, find the causal condition that led to that state. For example, given measurements of the acoustic pressures in the ocean at some time instant, find the source that started emitting the acoustic sounds. The inverse problem is often considered more challenging since one has access to limited data (for example, recordings at a small set of sensors only), the data may be noisy, some recordings may be missing, etc. Inverse problems are often ill-posed, meaning they do not necessarily have a solution and if so, it may not necessarily be unique. In this paper we focus on inverse problems. The main applications involve recovering the original state of a physical system given partial information from future states. There are many different physical experiments that can be mathematically formulated as inverse problems, such as inverse scattering \cite{}, source refocusing \cite{}, material identification \cite{}, non-destructive testing \cite{}, and many more which serve as motivation for this work.

Most latest advances of artificial intelligence involve deep neural networks \cite{}. Due to their ability to fit non-linear problems with high accuracy and generalize, as well as the availability of diverse architectures to fit a variety of tasks, they have been used in many applications. One drawback is the training time and resources it takes to train the networks, hence more efficient architectures are highly sought after. A recent innovation in the field are the so-called transformers \cite{}, which refer to deep neural networks that have an attention mechanism \cite{}. The attention module attempts to understand context from the given input. To learn the context, the attention mechanism operates on a discrete embedding of the data that is composed of tokens. An immediate example is Natural Language Programming (NLP) using transformers, where a sentence is embedded using tokens according to a specific vocabulary \cite{}.

A challenge that arises when using transformers is considering non-discrete data. For example, instead of sentences (sequence of words), we would like to embed a continuous function or signal. The literature offers methods to achieve that, as introduced in the following section. One prominent method, explored in this work, is called Vision Transformers (ViT) \cite{}. The vision transformers receive an image as input, for example the initial condition of a system (in the forward problem), or a future state of a system (in the inverse problem). Then, the image is split into small regions, and each region acts as a token. The vision transformer extracts the context from the tokens (regions of the image), and thus is able to utilize the attention mechanism for the continuous signal and make accurate predictions.

Another key component of this work is operator learning. Machine learning models aim to find a function that connects input data to output data. Operators train to represent mappings from a family of functions to another family of functions. For example, if one wants to infer the acoustic wave pressure in the ocean for each and every initial source, they can define the operator as the mapping from the initial source (a function, initial pressure in every point of the domain) to the pressures at a later time (also a function, future pressures in every point of the domain). The main advantage of operator learning is that, after the operator has been learned, no further training is needed and the solution e.g. for a partial differential equation (PDE), which can be very expensive using classic methods, can be simply inferred (estimated) by the network with low computational cost.

In this paper we combine vision transformers with operator learning to solve a variety of inverse problems. We propose a U-net \cite{} based architecture, infused with a ViT, to do operator learning. The operators in this case solve inverse problems that are of high interest in the scientific community. We show that the results using the proposed method exceed expectations, beating the leading operator network benchmarks in terms of accuracy. In addition, the transformers require much less data and the architecture is lighter (less parameters to train), achieving up to 5.5 times faster computation time.

